The miniJPAS & J-NEP surveys: Identification and characterization of the Ly$\alpha$ Emitter population and the Ly$\alpha$ Luminosity Function

We present the Lyman-$a$ (Lya) Luminosity Function (LF) at $2.05<z<3.75$, estimated from a sample of 67 Lya-emitter (LAE) candidates in the J-PAS Pathfinder surveys: miniJPAS and J-NEP. These two surveys cover a total effective area of $\sim 1.14$ deg$^2$ with 54 Narrow Band (NB) filters across the optical range, with typical limiting magnitudes of $\sim 23$. This set of NBs allows to probe Lya emission in a wide and continuous range of redshifts. We develop a method for detecting Lya emission for the estimation of the Lya LF using the whole J-PAS filter set. We test this method by applying it to the miniJPAS and J-NEP data. In order to compute the corrections needed to estimate the Lya LF and to test the performance of the candidates selection method, we build mock catalogs. These include representative populations of Lya Emitters at $1.9<z<4.5$ as well as their expected contaminants, namely low-$z$ galaxies and $z<2$ QSOs. We show that our method is able to provide the Lya LF at the intermediate-bright range of luminosity ($\rm 10^{43.5} erg\,s^{-1} \lesssim L_{Lya} \lesssim 10^{44.5} erg\,s^{-1}$). The photometric information provided by these surveys suggests that our samples are dominated by bright, Lya-emitting Active Galactic Nuclei. At $L_{{\rm Ly}a}<10^{44.5}$ erg\,s$^{-1}$, we fit our Lya LF to a power-law with slope $A=0.70\pm0.25$. We also fit a Schechter function to our data, obtaining: Log$(\Phi^* / \text{Mpc$^{-3}$})=-6.30^{+0.48}_{-0.70}$, Log$(L^*/ \rm erg\,s^{-1})=44.85^{+0.50}_{-0.32}$, $a=-1.65^{+0.29}_{-0.27}$. Overall, our results confirm the presence of an AGN component at the bright-end of the Lya LF. In particular, we find no significant contribution of star-forming LAEs to the Lya LF at Log$(L_{\rm Lya}$ / erg s$^{-1}$)>43.5. This work serves as a proof-of-concept for the results that can be obtained with the upcoming data releases of the J-PAS survey.

==> appendices.tex <==
\appendix

\section{Candidates catalog}

Table \ref{tab:selected_catalog} lists the 91 candidates selected by our method as LAEs, containing only the sources with \texttt{morph\_prob\_star} < 0.1, as explained in { Sect.}~\ref{sec:LAEs_morph}. This entire catalog is representative of what can be directly obtained of any J-PAS data set. The sources used in the Ly$\alpha$ LF estimation are marked in blue. As explained in Sect. \ref{sec:visual_inspection}, the sub-sample of objects used for the Ly$\alpha$ LF are chosen after a visual inspection and cross-matches with SDSS DR16 and HETDEX Source Catalog 1.

The description of each column is the following:
\begin{itemize}
    \item Field: The sub-field of miniJPAS or J-NEP in which the source was detected by \texttt{SExtractor}.
    \item tile\_id: The ID identifying the selection tile of miniJPAS or J-NEP.
    \item number: Unique ID of each object within each tile in the dual-mode catalogs of miniJPAS or J-NEP.
    \item RA, DEC: Right ascension and declination.
    \item $z_\mathrm{NB}$: Ly$\alpha$ redshift of the central wavelength of the line detection. The provided error is inferred from the FWHM of the NB.
    \item Selected NB: Name of the NB of the Ly$\alpha$ line detection.
    \item SDSS spCL, SDSS $z_\mathrm{spec}$: Spectroscopic class and redshift of the counterpart in SDSS DR16.
    \item HETDEX spCl, HETDEX $z_\mathrm{spec}$: Spectroscopic class and redshift of the counterpart in HETDEX Source Catalog 1.
    \item VI class: Class assigned in the visual inspection (see Sect. \ref{sec:visual_inspection})
    \item $\log_{10}L_{\mathrm{Ly}\alpha}$: Estimated Ly$\alpha$ luminosity.
    \item EW$_0^{\mathrm{Ly}\alpha}$: Estimated rest-frame EW of the Ly$\alpha$ line.
    \item $P^\mathrm{2D}$: Purity extracted from the 2D correction maps according to the source $L_{\mathrm{Ly}\alpha}$ and $r$ magnitude (see Sect. \ref{sec:2dpuricomp}). This value can be seen as the probability of each source to be a true positive LAE.
\end{itemize}


\input{selection_table.tex}


\section{2D purity and number count corrections}\label{app:2dmaps}

In Fig.~\ref{fig:2dpuricomp} we show example representations of the 2D correction maps described in Sect.~\ref{sec:2dpuricomp}, for $2.3<z<2.8$. These maps are computed for every redshift interval used in this work, for every field of miniJPAS and J-NEP. { The non-colored regions in Fig.~\ref{fig:2dpuricomp} correspond to combinations of parameters incompatible with the LAEs of our mock, thus the candidates laying in this areas of the 2D map are assigned $P^\mathrm{2D}=w^\mathrm{2D}=0$}.

\begin{figure*}
    \centering
    \begin{subfigure}{0.485\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/PuriComp2D_minijpasAEGIS001.pdf}
    \caption{AEGIS001}
    \end{subfigure}
    \begin{subfigure}{0.485\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/PuriComp2D_minijpasAEGIS002.pdf}
    \caption{AEGIS002}
    \end{subfigure}
    \begin{subfigure}{0.485\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/PuriComp2D_minijpasAEGIS003.pdf}
    \caption{AEGIS003}
    \end{subfigure}
    \begin{subfigure}{0.485\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/PuriComp2D_minijpasAEGIS004.pdf}
    \caption{AEGIS004}
    \end{subfigure}
    \begin{subfigure}{0.485\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/PuriComp2D_jnep.pdf}
    \caption{J-NEP}
    \end{subfigure}
        
    \caption{2D maps of the purity and number count correction for the four miniJPAS fields and J-NEP in the redshift interval $z=2.3$--$2.8$. The maps are computed for every field in miniJPAS and J-NEP and every interval of redshift used in this work, only one $z$ interval is shown for brevity. The black squares and error bars represent the LAE candidates of each field in the chosen interval of redshift.}
    \label{fig:2dpuricomp}
\end{figure*}

\section{Purity calibration}\label{sec:prior_LF_choice}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/rho_LF_puri_one.pdf}
    \caption{Effects of varying the sample purity on the estimated Ly$\alpha$ LF. {Top:} Colored squares show different realizations of our Ly$\alpha$ LF in the range $z=2.0-3.8$, obtained after scaling the number of true positives in the purity computation by a factor $\rho=0.1, 0.5, 1.0, 1.5, 2.0$. We also show the mock QSO LF for each $\rho$ (solid lines). We show the uncertainties of the LF with $\rho=1$. The variation of the LF is inside the $1\sigma$ errors for all the shown values of $\rho$. { Bottom: Estimated purity for the different values of $\rho$.}}
    \label{fig:rho_LF}
\end{figure}

As introduced in Sect. \ref{sec:mocks}, the corrections of our LF are likely to be biased by the underlying luminosity distribution we impose to our mock data. The number count correction estimate does not depend on the parameter space distribution of the mocks, as it is only a measure on how likely is to select a source as a function of its intrinsic $L_{\mathrm{Ly}\alpha}$ and EW. Nonetheless, the purity estimate is strongly dependent on the relative abundances of the objects from the target population in relation to that of the contaminants.

To check the robustness of our corrections in the QSO regime, we alter the purity estimate by introducing a factor $\rho$ to the true positive count. We recalculate the 2D purity as
\begin{equation}
    p^\mathrm{2D}=\frac{\rho\cdot\text{TP}}{\rho\cdot\text{TP} + \text{FP}} ,
\end{equation}
and compute the Ly$\alpha$ LF of miniJPAS\&J-NEP, using this new definition of the purity, for different values of $\rho$. Since the effect of increasing/decreasing the value of $\rho$ is equivalent to increasing/decreasing the mock QSO { number density}, this procedure tests the effect of under/overestimating the purity of our selected sample. We estimate the Ly$\alpha$ LF for different values of $\rho$ using the whole selected sample of 127 candidates (see Sec. \ref{sec:LAEs_cat}). The upper panel of Fig. \ref{fig:rho_LF} shows the recomputed LFs for different values of $\rho$ (as detailed by the plot label). Solid lines show the resulting $L_{\mathrm{Ly}\alpha}$ distribution of our QSO mock, for each $\rho$ value. The comparison between the different LF realizations (colored squares and error-bars) show that the change produced onto the LF by varying $\rho$ is small, especially when compared to the $1\sigma$ uncertainties for the $\rho=1$ realization (black error bars). In addition, the value of $\rho$ that produces an input LF comparable to the estimated is close to $\rho\sim 1$. With the eventual release of larger catalog of J-PAS, it will be possible to accurately calibrate the purity of the LAE candidate sample.

As already discussed in Sect. \ref{sec:qso_frac}, our LAE candidate sample is expected to be vastly dominated by AGN. Consequently, any change in the prior LF used for the construction of the SFG mock produces a minimum change onto our final results. Although we predict a non-zero contribution of SFG in our sample, the observational data is insufficient for calibrating the purity at the SFG regime ($\log_{10}(L_{\mathrm{Ly}\alpha} / \mathrm{erg\,s}^{-1})\lesssim 43.5$) with the current selection method.

==> fit_params_table.tex <==
\begin{table*}
    \centering
    \caption{caption}
    \label{tab:N_sel}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cc|c|ccccccc}
    \toprule

    

    \bottomrule
    \end{tabular}
    }
\end{table*}

==> selection_table_old.tex <==
\setlength\LTleft{0pt}
\setlength\LTright{0pt}
\begin{longtable}{ccccccccccccccc}
\toprule
Field & tile\textunderscore id & number & RA & DEC & \makecell{$z_\text{NB}$ \\ $(\pm 0.04)$} & Sel. NB & \makecell{SDSS \\ SpCl} & \makecell{SDSS \\ $z_\text{spec}$} & \makecell{HETDEX \\ SpCl} & \makecell{HETDEX \\ $z_\mathrm{spec}$} & VI class & \makecell{$\logten\Llya$ \\ (erg\,s$^{-1}$)} & \makecell{EW$_0^{\mathrm{Ly}\alpha}$ \\ (\AA)} & $P(\text{LAE})$\\
\midrule
AEGIS001 & 2241 & 468 & 14h15m42.2s & 52\degr22\arcmin7.0\arcsec & 2.11 & J0378 & QSO & 1.00 & agn & 1.00 & Cont. QSO & 43.69$^{ + 0.11}_{ - 0.14}$ & 62$\pm$10 & 0.00 \\ 
\color{blue}AEGIS001 & \color{blue}2241 & \color{blue}9344 & \color{blue}14h17m38.8s & \color{blue}52\degr23\arcmin33.1\arcsec & \color{blue}2.11 & \color{blue}J0378 & \color{blue}QSO & \color{blue}2.16 & \color{blue}agn & \color{blue}2.16 & \color{blue}QSO LAE & \color{blue}44.11$^{ + 0.06}_{ - 0.07}$ & \color{blue}184$\pm$13 & \color{blue}1.00 \\ 
\color{blue}AEGIS001 & \color{blue}2241 & \color{blue}11097 & \color{blue}14h18m42.3s & \color{blue}52\degr36\arcmin43.9\arcsec & \color{blue}2.11 & \color{blue}J0378 & \color{blue}QSO & \color{blue}2.12 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.63$^{ + 0.12}_{ - 0.16}$ & \color{blue}93$\pm$16 & \color{blue}0.98 \\ 
AEGIS001 & 2241 & 13090 & 14h16m58.4s & 52\degr48\arcmin6.3\arcsec & 2.11 & J0378 & QSO & 1.96 & - & - & Cont. QSO & 43.73$^{ + 0.10}_{ - 0.13}$ & 37$\pm$6 & 0.00 \\ 
AEGIS001 & 2241 & 14254 & 14h18m2.0s & 52\degr35\arcmin14.9\arcsec & 2.11 & J0378 & QSO & 1.49 & - & - & Cont. QSO & 43.92$^{ + 0.07}_{ - 0.09}$ & 37$\pm$4 & 0.00 \\ 
\color{blue}AEGIS001 & \color{blue}2241 & \color{blue}17351 & \color{blue}14h18m32.8s & \color{blue}52\degr23\arcmin50.0\arcsec & \color{blue}2.11 & \color{blue}J0378 & \color{blue}QSO & \color{blue}2.04 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.83$^{ + 0.08}_{ - 0.10}$ & \color{blue}42$\pm$5 & \color{blue}0.87 \\ 
AEGIS001 & 2241 & 18457 & 14h17m36.0s & 52\degr30\arcmin29.8\arcsec & 2.11 & J0378 & QSO & 0.99 & - & - & Cont. QSO & 43.62$^{ + 0.12}_{ - 0.17}$ & 43$\pm$8 & 0.00 \\ 
AEGIS001 & 2241 & 19989 & 14h19m11.4s & 52\degr32\arcmin34.7\arcsec & 2.11 & J0378 & QSO & 1.41 & - & - & Cont. QSO & 43.44$^{ + 0.16}_{ - 0.26}$ & 73$\pm$19 & 0.00 \\ 
AEGIS001 & 2241 & 13288 & 14h17m37.3s & 52\degr42\arcmin36.7\arcsec & 2.21 & J0390 & QSO & 0.15 & - & - & Cont. QSO & 43.10$^{ + 0.14}_{ - 0.21}$ & 42$\pm$9 & 0.00 \\ 
AEGIS001 & 2241 & 14038 & 14h18m42.9s & 52\degr29\arcmin19.0\arcsec & 2.21 & J0390 & QSO & 1.08 & - & - & Cont. QSO & 43.07$^{ + 0.15}_{ - 0.23}$ & 55$\pm$13 & 0.00 \\ 
AEGIS001 & 2241 & 15333 & 14h18m13.1s & 52\degr31\arcmin10.1\arcsec & 2.21 & J0390 & - & - & - & - & Low-$z$ Gal. & 43.04$^{ + 0.16}_{ - 0.25}$ & 74$\pm$18 & 0.00 \\ 
AEGIS001 & 2241 & 15615 & 14h17m23.9s & 52\degr38\arcmin6.0\arcsec & 2.21 & J0390 & QSO & 1.52 & - & - & Cont. QSO & 43.79$^{ + 0.05}_{ - 0.06}$ & 50$\pm$3 & 0.00 \\ 
AEGIS001 & 2241 & 15867 & 14h18m16.2s & 52\degr29\arcmin40.7\arcsec & 2.29 & J0400 & QSO & 1.61 & - & - & Cont. QSO & 44.10$^{ + 0.05}_{ - 0.05}$ & 44$\pm$2 & 0.00 \\ 
AEGIS001 & 2241 & 4536 & 14h16m19.6s & 52\degr24\arcmin58.8\arcsec & 2.46 & J0420 & - & - & - & - & Low-$z$ Gal. & 43.47$^{ + 0.15}_{ - 0.23}$ & 66$\pm$16 & 0.00 \\ 
\color{blue}AEGIS001 & \color{blue}2241 & \color{blue}8524 & \color{blue}14h16m25.5s & \color{blue}52\degr32\arcmin42.6\arcsec & \color{blue}2.54 & \color{blue}J0430 & \color{blue}- & \color{blue}- & \color{blue}agn & \color{blue}2.56 & \color{blue}QSO LAE & \color{blue}43.93$^{ + 0.05}_{ - 0.05}$ & \color{blue}71$\pm$4 & \color{blue}0.99 \\ 
AEGIS001 & 2241 & 20770 & 14h18m23.3s & 52\degr40\arcmin4.6\arcsec & 2.54 & J0430 & QSO & 1.77 & - & - & Cont. QSO & 44.13$^{ + 0.04}_{ - 0.05}$ & 91$\pm$3 & 0.00 \\ 
\color{blue}AEGIS001 & \color{blue}2241 & \color{blue}4481 & \color{blue}14h17m23.1s & \color{blue}52\degr15\arcmin14.7\arcsec & \color{blue}2.62 & \color{blue}J0440 & \color{blue}QSO & \color{blue}2.59 & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}44.16$^{ + 0.05}_{ - 0.05}$ & \color{blue}43$\pm$2 & \color{blue}1.00 \\ 
AEGIS001 & 2241 & 2717 & 14h16m50.0s & 52\degr16\arcmin40.2\arcsec & 2.70 & J0450 & - & - & - & - & Low-$z$ Gal. & 43.79$^{ + 0.14}_{ - 0.21}$ & 53$\pm$13 & 0.00 \\ 
\color{blue}AEGIS001 & \color{blue}2241 & \color{blue}7775 & \color{blue}14h16m9.0s & \color{blue}52\degr33\arcmin23.1\arcsec & \color{blue}2.79 & \color{blue}J0460 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.23$^{ + 0.14}_{ - 0.20}$ & \color{blue}96$\pm$21 & \color{blue}0.95 \\ 
\color{blue}AEGIS001 & \color{blue}2241 & \color{blue}14404 & \color{blue}14h17m35.3s & \color{blue}52\degr38\arcmin51.4\arcsec & \color{blue}2.79 & \color{blue}J0460 & \color{blue}QSO & \color{blue}1.96 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}44.43$^{ + 0.04}_{ - 0.04}$ & \color{blue}66$\pm$1 & \color{blue}0.97 \\ 
\color{blue}AEGIS001 & \color{blue}2241 & \color{blue}15255 & \color{blue}14h17m47.3s & \color{blue}52\degr35\arcmin10.6\arcsec & \color{blue}2.79 & \color{blue}J0460 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}43.57$^{ + 0.08}_{ - 0.09}$ & \color{blue}81$\pm$8 & \color{blue}0.91 \\ 
\color{blue}AEGIS001 & \color{blue}2241 & \color{blue}15524 & \color{blue}14h16m51.6s & \color{blue}52\degr43\arcmin12.4\arcsec & \color{blue}2.79 & \color{blue}J0460 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.19$^{ + 0.15}_{ - 0.23}$ & \color{blue}53$\pm$13 & \color{blue}0.83 \\ 
\color{blue}AEGIS001 & \color{blue}2241 & \color{blue}6762 & \color{blue}14h17m42.0s & \color{blue}52\degr17\arcmin7.3\arcsec & \color{blue}2.87 & \color{blue}J0470 & \color{blue}- & \color{blue}- & \color{blue}agn & \color{blue}2.06 & \color{blue}- & \color{blue}43.44$^{ + 0.13}_{ - 0.19}$ & \color{blue}90$\pm$18 & \color{blue}0.89 \\ 
\color{blue}AEGIS001 & \color{blue}2241 & \color{blue}20626 & \color{blue}14h18m40.6s & \color{blue}52\degr37\arcmin16.4\arcsec & \color{blue}2.87 & \color{blue}J0470 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.49$^{ + 0.12}_{ - 0.16}$ & \color{blue}49$\pm$9 & \color{blue}0.84 \\ 
\color{blue}AEGIS001 & \color{blue}2241 & \color{blue}4983 & \color{blue}14h16m15.3s & \color{blue}52\degr26\arcmin26.5\arcsec & \color{blue}2.95 & \color{blue}J0480 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.52$^{ + 0.13}_{ - 0.18}$ & \color{blue}47$\pm$9 & \color{blue}0.57 \\ 
\color{blue}AEGIS001 & \color{blue}2241 & \color{blue}20297 & \color{blue}14h18m9.7s & \color{blue}52\degr43\arcmin0.2\arcsec & \color{blue}3.19 & \color{blue}J0510 & \color{blue}QSO & \color{blue}3.19 & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}44.17$^{ + 0.04}_{ - 0.05}$ & \color{blue}73$\pm$4 & \color{blue}0.98 \\ 
\color{blue}AEGIS001 & \color{blue}2241 & \color{blue}5837 & \color{blue}14h16m11.9s & \color{blue}52\degr28\arcmin44.5\arcsec & \color{blue}3.28 & \color{blue}J0520 & \color{blue}QSO & \color{blue}3.25 & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}43.95$^{ + 0.12}_{ - 0.17}$ & \color{blue}68$\pm$13 & \color{blue}1.00 \\ 
\color{blue}AEGIS001 & \color{blue}2241 & \color{blue}14553 & \color{blue}14h17m55.3s & \color{blue}52\degr35\arcmin32.8\arcsec & \color{blue}3.36 & \color{blue}J0530 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.47$^{ + 0.12}_{ - 0.16}$ & \color{blue}164$\pm$27 & \color{blue}0.91 \\ 
\color{blue}AEGIS001 & \color{blue}2241 & \color{blue}9742 & \color{blue}14h16m25.3s & \color{blue}52\degr35\arcmin38.3\arcsec & \color{blue}3.60 & \color{blue}J0560 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}44.07$^{ + 0.08}_{ - 0.09}$ & \color{blue}377$\pm$38 & \color{blue}0.98 \\ 
\color{blue}AEGIS001 & \color{blue}2241 & \color{blue}13746 & \color{blue}14h17m24.2s & \color{blue}52\degr41\arcmin50.8\arcsec & \color{blue}3.69 & \color{blue}J0570 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}44.02$^{ + 0.08}_{ - 0.10}$ & \color{blue}88$\pm$10 & \color{blue}0.97 \\ 
\color{blue}AEGIS002 & \color{blue}2243 & \color{blue}2395 & \color{blue}14h18m18.5s & \color{blue}52\degr43\arcmin56.1\arcsec & \color{blue}2.11 & \color{blue}J0378 & \color{blue}QSO & \color{blue}2.14 & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}43.92$^{ + 0.06}_{ - 0.08}$ & \color{blue}131$\pm$12 & \color{blue}1.00 \\ 
\color{blue}AEGIS002 & \color{blue}2243 & \color{blue}5085 & \color{blue}14h19m18.1s & \color{blue}52\degr41\arcmin58.4\arcsec & \color{blue}2.11 & \color{blue}J0378 & \color{blue}QSO & \color{blue}2.03 & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}43.99$^{ + 0.06}_{ - 0.07}$ & \color{blue}64$\pm$5 & \color{blue}0.98 \\ 
\color{blue}AEGIS002 & \color{blue}2243 & \color{blue}4295 & \color{blue}14h18m14.3s & \color{blue}52\degr49\arcmin13.1\arcsec & \color{blue}2.21 & \color{blue}J0390 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.14$^{ + 0.17}_{ - 0.29}$ & \color{blue}67$\pm$19 & \color{blue}0.89 \\ 
\color{blue}AEGIS002 & \color{blue}2243 & \color{blue}7958 & \color{blue}14h20m16.8s & \color{blue}52\degr42\arcmin2.8\arcsec & \color{blue}2.21 & \color{blue}J0390 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.29$^{ + 0.13}_{ - 0.18}$ & \color{blue}150$\pm$29 & \color{blue}1.00 \\ 
\color{blue}AEGIS002 & \color{blue}2243 & \color{blue}7718 & \color{blue}14h19m29.0s & \color{blue}52\degr49\arcmin59.3\arcsec & \color{blue}2.29 & \color{blue}J0400 & \color{blue}- & \color{blue}- & \color{blue}agn & \color{blue}2.31 & \color{blue}QSO LAE & \color{blue}43.60$^{ + 0.10}_{ - 0.13}$ & \color{blue}162$\pm$23 & \color{blue}1.00 \\ 
AEGIS002 & 2243 & 15119 & 14h20m16.0s & 52\degr51\arcmin1.3\arcsec & 2.29 & J0400 & QSO & 1.62 & - & - & Cont. QSO & 43.78$^{ + 0.07}_{ - 0.09}$ & 96$\pm$10 & 0.00 \\ 
\color{blue}AEGIS002 & \color{blue}2243 & \color{blue}12352 & \color{blue}14h19m52.8s & \color{blue}53\degr2\arcmin4.2\arcsec & \color{blue}2.70 & \color{blue}J0450 & \color{blue}QSO & \color{blue}1.90 & \color{blue}agn & \color{blue}1.90 & \color{blue}- & \color{blue}44.29$^{ + 0.06}_{ - 0.08}$ & \color{blue}52$\pm$4 & \color{blue}1.00 \\ 
\color{blue}AEGIS002 & \color{blue}2243 & \color{blue}14558 & \color{blue}14h19m26.8s & \color{blue}53\degr0\arcmin3.5\arcsec & \color{blue}2.95 & \color{blue}J0480 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.75$^{ + 0.13}_{ - 0.19}$ & \color{blue}59$\pm$13 & \color{blue}0.97 \\ 
\color{blue}AEGIS002 & \color{blue}2243 & \color{blue}4755 & \color{blue}14h19m23.1s & \color{blue}52\degr40\arcmin13.4\arcsec & \color{blue}3.03 & \color{blue}J0490 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.85$^{ + 0.12}_{ - 0.17}$ & \color{blue}50$\pm$10 & \color{blue}0.99 \\ 
\color{blue}AEGIS002 & \color{blue}2243 & \color{blue}5404 & \color{blue}14h18m13.4s & \color{blue}52\degr52\arcmin40.0\arcsec & \color{blue}3.28 & \color{blue}J0520 & \color{blue}QSO & \color{blue}3.29 & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}44.40$^{ + 0.06}_{ - 0.07}$ & \color{blue}140$\pm$9 & \color{blue}1.00 \\ 
\color{blue}AEGIS002 & \color{blue}2243 & \color{blue}14873 & \color{blue}14h19m35.6s & \color{blue}52\degr57\arcmin10.7\arcsec & \color{blue}3.28 & \color{blue}J0520 & \color{blue}QSO & \color{blue}3.22 & \color{blue}agn & \color{blue}3.22 & \color{blue}QSO LAE & \color{blue}44.54$^{ + 0.05}_{ - 0.05}$ & \color{blue}83$\pm$4 & \color{blue}1.00 \\ 
\color{blue}AEGIS002 & \color{blue}2243 & \color{blue}673 & \color{blue}14h19m14.3s & \color{blue}52\degr30\arcmin50.3\arcsec & \color{blue}3.43 & \color{blue}J0540 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.86$^{ + 0.10}_{ - 0.12}$ & \color{blue}134$\pm$20 & \color{blue}0.95 \\ 
\color{blue}AEGIS002 & \color{blue}2243 & \color{blue}5769 & \color{blue}14h17m56.9s & \color{blue}52\degr56\arcmin15.4\arcsec & \color{blue}3.43 & \color{blue}J0540 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.75$^{ + 0.12}_{ - 0.16}$ & \color{blue}63$\pm$11 & \color{blue}0.90 \\ 
\color{blue}AEGIS002 & \color{blue}2243 & \color{blue}15610 & \color{blue}14h19m43.6s & \color{blue}52\degr54\arcmin31.3\arcsec & \color{blue}3.43 & \color{blue}J0540 & \color{blue}QSO & \color{blue}3.44 & \color{blue}agn & \color{blue}3.44 & \color{blue}QSO LAE & \color{blue}44.52$^{ + 0.04}_{ - 0.04}$ & \color{blue}191$\pm$6 & \color{blue}0.99 \\ 
AEGIS003 & 2406 & 6731 & 14h22m5.7s & 53\degr10\arcmin54.1\arcsec & 2.21 & J0390 & QSO & 1.45 & - & - & Cont. QSO & 43.30$^{ + 0.13}_{ - 0.20}$ & 39$\pm$8 & 0.00 \\ 
\color{blue}AEGIS003 & \color{blue}2406 & \color{blue}1224 & \color{blue}14h21m18.0s & \color{blue}52\degr53\arcmin46.0\arcsec & \color{blue}2.29 & \color{blue}J0400 & \color{blue}QSO & \color{blue}2.31 & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}44.36$^{ + 0.05}_{ - 0.05}$ & \color{blue}109$\pm$4 & \color{blue}1.00 \\ 
\color{blue}AEGIS003 & \color{blue}2406 & \color{blue}1482 & \color{blue}14h20m6.0s & \color{blue}53\degr5\arcmin9.4\arcsec & \color{blue}2.46 & \color{blue}J0420 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.69$^{ + 0.14}_{ - 0.21}$ & \color{blue}67$\pm$16 & \color{blue}0.99 \\ 
AEGIS003 & 2406 & 7049 & 14h20m43.7s & 53\degr22\arcmin6.3\arcsec & 2.46 & J0420 & QSO & 1.72 & - & - & Cont. QSO & 44.45$^{ + 0.05}_{ - 0.06}$ & 54$\pm$2 & 0.00 \\ 
\color{blue}AEGIS003 & \color{blue}2406 & \color{blue}11608 & \color{blue}14h23m6.1s & \color{blue}53\degr15\arcmin29.0\arcsec & \color{blue}2.46 & \color{blue}J0420 & \color{blue}QSO & \color{blue}2.46 & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}45.00$^{ + 0.04}_{ - 0.05}$ & \color{blue}71$\pm$1 & \color{blue}1.00 \\ 
\color{blue}AEGIS003 & \color{blue}2406 & \color{blue}6169 & \color{blue}14h20m46.4s & \color{blue}53\degr12\arcmin24.5\arcsec & \color{blue}2.54 & \color{blue}J0430 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}43.86$^{ + 0.08}_{ - 0.10}$ & \color{blue}90$\pm$11 & \color{blue}0.99 \\ 
\color{blue}AEGIS003 & \color{blue}2406 & \color{blue}14091 & \color{blue}14h21m32.5s & \color{blue}53\degr22\arcmin44.2\arcsec & \color{blue}2.54 & \color{blue}J0430 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.56$^{ + 0.13}_{ - 0.20}$ & \color{blue}81$\pm$17 & \color{blue}0.99 \\ 
\color{blue}AEGIS003 & \color{blue}2406 & \color{blue}4342 & \color{blue}14h20m10.5s & \color{blue}53\degr12\arcmin23.9\arcsec & \color{blue}2.62 & \color{blue}J0440 & \color{blue}QSO & \color{blue}2.59 & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}44.31$^{ + 0.04}_{ - 0.05}$ & \color{blue}56$\pm$2 & \color{blue}0.99 \\ 
AEGIS003 & 2406 & 4658 & 14h20m25.6s & 53\degr11\arcmin5.2\arcsec & 2.62 & J0440 & QSO & 1.85 & - & - & Cont. QSO & 43.50$^{ + 0.12}_{ - 0.17}$ & 62$\pm$11 & 0.00 \\ 
\color{blue}AEGIS003 & \color{blue}2406 & \color{blue}3657 & \color{blue}14h20m18.8s & \color{blue}53\degr9\arcmin11.3\arcsec & \color{blue}2.79 & \color{blue}J0460 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}43.74$^{ + 0.07}_{ - 0.08}$ & \color{blue}114$\pm$11 & \color{blue}0.92 \\ 
\color{blue}AEGIS003 & \color{blue}2406 & \color{blue}8977 & \color{blue}14h21m13.3s & \color{blue}53\degr12\arcmin18.6\arcsec & \color{blue}2.79 & \color{blue}J0460 & \color{blue}QSO & \color{blue}1.95 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}44.07$^{ + 0.04}_{ - 0.05}$ & \color{blue}55$\pm$3 & \color{blue}0.97 \\ 
\color{blue}AEGIS003 & \color{blue}2406 & \color{blue}11219 & \color{blue}14h21m60.0s & \color{blue}53\degr26\arcmin9.2\arcsec & \color{blue}2.79 & \color{blue}J0460 & \color{blue}QSO & \color{blue}2.73 & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}44.08$^{ + 0.05}_{ - 0.05}$ & \color{blue}47$\pm$3 & \color{blue}0.99 \\ 
\color{blue}AEGIS003 & \color{blue}2406 & \color{blue}14869 & \color{blue}14h21m36.5s & \color{blue}53\degr20\arcmin14.2\arcsec & \color{blue}2.87 & \color{blue}J0470 & \color{blue}QSO & \color{blue}2.02 & \color{blue}agn & \color{blue}2.02 & \color{blue}QSO LAE & \color{blue}43.89$^{ + 0.07}_{ - 0.09}$ & \color{blue}53$\pm$6 & \color{blue}0.95 \\ 
\color{blue}AEGIS003 & \color{blue}2406 & \color{blue}4964 & \color{blue}14h21m54.8s & \color{blue}52\degr58\arcmin41.9\arcsec & \color{blue}2.95 & \color{blue}J0480 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.84$^{ + 0.07}_{ - 0.09}$ & \color{blue}54$\pm$6 & \color{blue}0.91 \\ 
\color{blue}AEGIS003 & \color{blue}2406 & \color{blue}12752 & \color{blue}14h21m47.1s & \color{blue}53\degr24\arcmin5.8\arcsec & \color{blue}3.03 & \color{blue}J0490 & \color{blue}QSO & \color{blue}3.04 & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}44.40$^{ + 0.06}_{ - 0.06}$ & \color{blue}66$\pm$4 & \color{blue}0.99 \\ 
AEGIS004 & 2470 & 8781 & 14h15m51.6s & 52\degr0\arcmin25.6\arcsec & 2.21 & J0390 & QSO & 1.51 & - & - & Cont. QSO & 44.48$^{ + 0.05}_{ - 0.05}$ & 41$\pm$1 & 0.00 \\ 
\color{blue}AEGIS004 & \color{blue}2470 & \color{blue}2363 & \color{blue}14h15m11.8s & \color{blue}51\degr52\arcmin55.8\arcsec & \color{blue}2.29 & \color{blue}J0400 & \color{blue}QSO & \color{blue}2.31 & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}44.37$^{ + 0.05}_{ - 0.05}$ & \color{blue}57$\pm$2 & \color{blue}0.98 \\ 
\color{blue}AEGIS004 & \color{blue}2470 & \color{blue}4455 & \color{blue}14h13m47.9s & \color{blue}52\degr12\arcmin5.0\arcsec & \color{blue}2.38 & \color{blue}J0410 & \color{blue}QSO & \color{blue}2.35 & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}44.01$^{ + 0.07}_{ - 0.09}$ & \color{blue}97$\pm$11 & \color{blue}1.00 \\ 
AEGIS004 & 2470 & 9749 & 14h13m47.7s & 52\degr16\arcmin46.3\arcsec & 2.38 & J0410 & QSO & 1.67 & - & - & Cont. QSO & 43.64$^{ + 0.16}_{ - 0.25}$ & 45$\pm$12 & 0.00 \\ 
\color{blue}AEGIS004 & \color{blue}2470 & \color{blue}13007 & \color{blue}14h14m59.3s & \color{blue}52\degr24\arcmin25.0\arcsec & \color{blue}2.38 & \color{blue}J0410 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}43.77$^{ + 0.11}_{ - 0.15}$ & \color{blue}127$\pm$23 & \color{blue}0.99 \\ 
\color{blue}AEGIS004 & \color{blue}2470 & \color{blue}3723 & \color{blue}14h14m28.2s & \color{blue}52\degr3\arcmin47.2\arcsec & \color{blue}2.70 & \color{blue}J0450 & \color{blue}QSO & \color{blue}2.69 & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}43.97$^{ + 0.10}_{ - 0.13}$ & \color{blue}87$\pm$15 & \color{blue}0.99 \\ 
AEGIS004 & 2470 & 13064 & 14h15m56.9s & 52\degr16\arcmin7.2\arcsec & 2.70 & J0450 & QSO & 1.39 & - & - & Cont. QSO & 43.87$^{ + 0.12}_{ - 0.17}$ & 47$\pm$10 & 0.00 \\ 
\color{blue}AEGIS004 & \color{blue}2470 & \color{blue}12623 & \color{blue}14h14m50.9s & \color{blue}52\degr26\arcmin40.4\arcsec & \color{blue}2.87 & \color{blue}J0470 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}43.52$^{ + 0.12}_{ - 0.17}$ & \color{blue}44$\pm$8 & \color{blue}0.89 \\ 
\color{blue}AEGIS004 & \color{blue}2470 & \color{blue}15095 & \color{blue}14h16m17.8s & \color{blue}52\degr7\arcmin18.3\arcsec & \color{blue}2.95 & \color{blue}J0480 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.77$^{ + 0.09}_{ - 0.11}$ & \color{blue}49$\pm$7 & \color{blue}0.88 \\ 
\color{blue}AEGIS004 & \color{blue}2470 & \color{blue}6481 & \color{blue}14h15m42.7s & \color{blue}52\degr9\arcmin27.2\arcsec & \color{blue}3.19 & \color{blue}J0510 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}44.01$^{ + 0.05}_{ - 0.06}$ & \color{blue}257$\pm$17 & \color{blue}0.98 \\ 
\color{blue}J-NEP & \color{blue}2520 & \color{blue}3222 & \color{blue}17h24m40.4s & \color{blue}65\degr35\arcmin0.2\arcsec & \color{blue}2.11 & \color{blue}J0378 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.58$^{ + 0.16}_{ - 0.27}$ & \color{blue}65$\pm$17 & \color{blue}0.94 \\ 
J-NEP & 2520 & 6815 & 17h23m43.8s & 65\degr40\arcmin32.8\arcsec & 2.11 & J0378 & - & - & - & - & Cont. QSO & 43.56$^{ + 0.17}_{ - 0.29}$ & 60$\pm$17 & 0.00 \\ 
J-NEP & 2520 & 9243 & 17h20m45.2s & 65\degr43\arcmin42.0\arcsec & 2.11 & J0378 & - & - & - & - & Cont. QSO & 43.66$^{ + 0.14}_{ - 0.22}$ & 50$\pm$12 & 0.00 \\ 
J-NEP & 2520 & 12771 & 17h23m14.1s & 65\degr47\arcmin46.2\arcsec & 2.11 & J0378 & QSO & 1.44 & - & - & Cont. QSO & 45.09$^{ + 0.05}_{ - 0.06}$ & 58$\pm$1 & 0.00 \\ 
J-NEP & 2520 & 22098 & 17h24m13.6s & 65\degr59\arcmin55.7\arcsec & 2.11 & J0378 & - & - & - & - & Cont. QSO & 44.29$^{ + 0.06}_{ - 0.07}$ & 37$\pm$2 & 0.00 \\ 
\color{blue}J-NEP & \color{blue}2520 & \color{blue}10356 & \color{blue}17h20m59.5s & \color{blue}65\degr44\arcmin57.8\arcsec & \color{blue}2.29 & \color{blue}J0400 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}43.72$^{ + 0.07}_{ - 0.09}$ & \color{blue}109$\pm$10 & \color{blue}0.99 \\ 
\color{blue}J-NEP & \color{blue}2520 & \color{blue}12539 & \color{blue}17h22m8.9s & \color{blue}65\degr47\arcmin43.1\arcsec & \color{blue}2.29 & \color{blue}J0400 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}44.09$^{ + 0.05}_{ - 0.06}$ & \color{blue}100$\pm$4 & \color{blue}1.00 \\ 
\color{blue}J-NEP & \color{blue}2520 & \color{blue}15690 & \color{blue}17h24m13.3s & \color{blue}65\degr55\arcmin28.8\arcsec & \color{blue}2.29 & \color{blue}J0400 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.30$^{ + 0.15}_{ - 0.23}$ & \color{blue}39$\pm$9 & \color{blue}0.93 \\ 
\color{blue}J-NEP & \color{blue}2520 & \color{blue}2518 & \color{blue}17h24m19.5s & \color{blue}65\degr33\arcmin59.7\arcsec & \color{blue}2.38 & \color{blue}J0410 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.55$^{ + 0.08}_{ - 0.10}$ & \color{blue}66$\pm$7 & \color{blue}0.98 \\ 
\color{blue}J-NEP & \color{blue}2520 & \color{blue}5302 & \color{blue}17h22m51.4s & \color{blue}65\degr38\arcmin20.5\arcsec & \color{blue}2.38 & \color{blue}J0410 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.33$^{ + 0.13}_{ - 0.19}$ & \color{blue}71$\pm$14 & \color{blue}0.97 \\ 
\color{blue}J-NEP & \color{blue}2520 & \color{blue}10708 & \color{blue}17h20m33.0s & \color{blue}65\degr45\arcmin18.7\arcsec & \color{blue}2.46 & \color{blue}J0420 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}44.13$^{ + 0.05}_{ - 0.06}$ & \color{blue}42$\pm$2 & \color{blue}0.98 \\ 
\color{blue}J-NEP & \color{blue}2520 & \color{blue}6012 & \color{blue}17h22m28.2s & \color{blue}65\degr39\arcmin23.5\arcsec & \color{blue}2.62 & \color{blue}J0440 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.22$^{ + 0.15}_{ - 0.23}$ & \color{blue}43$\pm$10 & \color{blue}0.93 \\ 
\color{blue}J-NEP & \color{blue}2520 & \color{blue}12726 & \color{blue}17h24m38.0s & \color{blue}65\degr47\arcmin48.6\arcsec & \color{blue}2.62 & \color{blue}J0440 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.23$^{ + 0.15}_{ - 0.23}$ & \color{blue}61$\pm$14 & \color{blue}0.96 \\ 
\color{blue}J-NEP & \color{blue}2520 & \color{blue}19539 & \color{blue}17h23m9.4s & \color{blue}65\degr50\arcmin13.7\arcsec & \color{blue}2.62 & \color{blue}J0440 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.18$^{ + 0.16}_{ - 0.25}$ & \color{blue}60$\pm$16 & \color{blue}0.91 \\ 
\color{blue}J-NEP & \color{blue}2520 & \color{blue}1652 & \color{blue}17h21m13.3s & \color{blue}65\degr32\arcmin45.2\arcsec & \color{blue}2.70 & \color{blue}J0450 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}43.85$^{ + 0.09}_{ - 0.12}$ & \color{blue}67$\pm$10 & \color{blue}0.99 \\ 
\color{blue}J-NEP & \color{blue}2520 & \color{blue}4903 & \color{blue}17h21m22.6s & \color{blue}65\degr37\arcmin45.3\arcsec & \color{blue}2.70 & \color{blue}J0450 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}44.22$^{ + 0.05}_{ - 0.06}$ & \color{blue}57$\pm$3 & \color{blue}0.99 \\ 
\color{blue}J-NEP & \color{blue}2520 & \color{blue}5247 & \color{blue}17h23m26.1s & \color{blue}65\degr38\arcmin16.3\arcsec & \color{blue}2.70 & \color{blue}J0450 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}44.20$^{ + 0.05}_{ - 0.06}$ & \color{blue}60$\pm$4 & \color{blue}0.99 \\ 
\color{blue}J-NEP & \color{blue}2520 & \color{blue}6520 & \color{blue}17h24m11.7s & \color{blue}65\degr40\arcmin4.7\arcsec & \color{blue}2.70 & \color{blue}J0450 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}43.66$^{ + 0.12}_{ - 0.17}$ & \color{blue}85$\pm$16 & \color{blue}0.99 \\ 
\color{blue}J-NEP & \color{blue}2520 & \color{blue}6636 & \color{blue}17h22m39.9s & \color{blue}65\degr40\arcmin17.1\arcsec & \color{blue}2.87 & \color{blue}J0470 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}43.55$^{ + 0.10}_{ - 0.14}$ & \color{blue}48$\pm$7 & \color{blue}0.92 \\ 
\color{blue}J-NEP & \color{blue}2520 & \color{blue}14925 & \color{blue}17h21m10.7s & \color{blue}65\degr56\arcmin27.4\arcsec & \color{blue}2.87 & \color{blue}J0470 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}44.48$^{ + 0.04}_{ - 0.04}$ & \color{blue}43$\pm$1 & \color{blue}0.98 \\ 
\color{blue}J-NEP & \color{blue}2520 & \color{blue}8395 & \color{blue}17h23m55.8s & \color{blue}65\degr42\arcmin46.0\arcsec & \color{blue}2.95 & \color{blue}J0480 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}QSO LAE & \color{blue}43.76$^{ + 0.06}_{ - 0.08}$ & \color{blue}203$\pm$18 & \color{blue}0.86 \\ 
\color{blue}J-NEP & \color{blue}2520 & \color{blue}14697 & \color{blue}17h22m17.8s & \color{blue}66\degr0\arcmin3.9\arcsec & \color{blue}3.60 & \color{blue}J0560 & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}- & \color{blue}44.08$^{ + 0.08}_{ - 0.09}$ & \color{blue}127$\pm$13 & \color{blue}1.00 \\ 
\bottomrule
\caption{Catalog of sources selected as LAEs.}
\label{tab:selected_catalog}
\end{longtable}
